GPT-4V Takes the Wheel: Promises and Challenges for Pedestrian Behavior Prediction

Predicting pedestrian behavior is the key to ensure safety and reliability of autonomous vehicles. While deep learning methods have been promising by learning from annotated video frame sequences, they often fail to fully grasp the dynamic interactions between pedestrians and traffic, crucial for accurate predictions. These models also lack nuanced common sense reasoning. Moreover, the manual annotation of datasets for these models is expensive and challenging to adapt to new situations. The advent of Vision Language Models (VLMs) introduces promising alternatives to these issues, thanks to their advanced visual and causal reasoning skills. To our knowledge, this research is the first to conduct both quantitative and qualitative evaluations of VLMs in the context of pedestrian behavior prediction for autonomous driving. We evaluate GPT-4V(ision) on publicly available pedestrian datasets: JAAD and WiDEVIEW. Our quantitative analysis focuses on GPT-4V's ability to predict pedestrian behavior in current and future frames. The model achieves a 57% accuracy in a zero-shot manner, which, while impressive, is still behind the state-of-the-art domain-specific models (70%) in predicting pedestrian crossing actions. Qualitatively, GPT-4V shows an impressive ability to process and interpret complex traffic scenarios, differentiate between various pedestrian behaviors, and detect and analyze groups. However, it faces challenges, such as difficulty in detecting smaller pedestrians and assessing the relative motion between pedestrians and the ego vehicle.

==> chats/boundingboxsize.tex <==
\subsubsection{The effect of pedestrian size} In this experiment, we assess the capability of GPT-4V in identifying pedestrian motion change with regard to the pedestrian size in the scene. To start with, we present ChatGPT-4V with two sets of image sequences extracted from video 160 of the JAAD dataset, each contains four key frames with 15 skipping frames apart and is labeled with sequential number in blue. The first sequence captures a further view of the interested pedestrian, while the second one presents a closer view where the pedestrian is bigger in the scene. Subsequently, we asked GPT-4V to describe the pedestrian behavior with the red box during this time period. When asked the same question, GPT-4V has difficulty detecting the pedestrian with the red box, thus giving false answers in describing the pedestrian's behavior in the first set of images. In contrast, it is able to provide a reasonable description of the pedestrian's behavior for the second set. This indicates that the bigger the pedestrian size in the scene, the better visual understanding the model might have, which aligns with the quantitative experiment results. 
\\
\begin{chatbox}[label=chat:bbox_size_jaad,title= Effect of pedestrian size on JAAD images]
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{chats/images/video_0160/0160.jpg}
\end{minipage}    
\end{flushright}
\begin{rightbubbles}
This is a time series of four pictures taken from a driving recorder. The chronological order is marked on the corresponding subfigure. As the driver of the car, please describe in detail the behavior of the pedestrian within red box on the left side of the image.
\end{rightbubbles}
\begin{leftbubbles}
The images you've provided appear to show a sequence of events as captured by a driving recorder. Here's a detailed description of the pedestrian's behavior within the red box on the left side of the image, as seen from the driver's perspective:

\begin{itemize}
    \item In the first image, the pedestrian is positioned on the sidewalk close to the curb. They seem to be looking towards the road, possibly assessing traffic before crossing.
    \item Moving to the second image, the pedestrian has taken a step forward, suggesting they are preparing to cross the street or have just begun to do so. Their attention is still directed towards the road, indicating awareness of the traffic conditions.
    \item In the third image, \textcolor{red}{the pedestrian is not visible}, which could mean that they have stepped out of the frame or possibly moved out of the line of sight of the camera.
    \item By the fourth image, \textcolor{red}{the pedestrian appears to have crossed the road and is now on the opposite sidewalk}, walking away from the roadway. This indicates they have successfully navigated across the street.
\end{itemize}
Throughout these images, it is clear that the pedestrian's behavior is focused on crossing the road safely.  
\end{leftbubbles}
% \begin{rightbubbles}
% In the fourth image, how do you know the pedestrian has crossed the road?   
% \end{rightbubbles}
% \begin{leftbubbles}
%  I apologize for the confusion in my previous message. Upon reexamining the fourth image, it is not possible to definitively conclude that the pedestrian has crossed the road because the pedestrian is not visible in the frame. Since the images provided do not show the pedestrian in the fourth image, any statement regarding their position would be speculative. It's important to only describe what is visible and evident in the images provided. Thank you for bringing this to my attention.
% \end{leftbubbles}



\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{chats/images/video_0160/0160_large.jpg}
\end{minipage}
\end{flushright}

\begin{rightbubbles}
This is a time series of four pictures taken from a driving recorder. The chronological order is marked on the corresponding subfigure. As the driver of the car, please describe in detail the behavior of the pedestrian within red box on the left side of the image.
\end{rightbubbles}
\begin{leftbubbles}
In the time series of images provided from a dashcam perspective, the pedestrian within the red box on the left side of the road exhibits the following behavior:
\begin{itemize}
    \item In the first image, the pedestrian has just stepped off the curb and is beginning to cross the road, seemingly outside of a designated crosswalk area.
    \item By the second image, the pedestrian has continued crossing and is now in the middle of the driving lane closest to the original curb, directly in the path of the oncoming vehicle (from which the photos are taken).
    \item In the third image, \textcolor{blue}{the pedestrian has moved further across, now reaching the median line of the road}, seemingly aware of the oncoming vehicle as they glance towards it.
    \item The fourth image shows \textcolor{blue}{the pedestrian having successfully crossed over the median line} and the adjacent lane, reaching the opposite side of the road.
\end{itemize}
Throughout the sequence, the pedestrian moves steadily across the street, from one side to the other, without any clear signs of hurrying or stopping, even as the vehicle approaches. It's important to note that the driver should exercise caution and be prepared to stop to allow the pedestrian to cross safely, especially since the pedestrian is not using a crosswalk.
\end{leftbubbles}
% \begin{rightbubbles}
% What are the essential clues for you to describe the pedestrian's behavior?  Like distance to curbs?
% \end{rightbubbles}
% \begin{leftbubbles}
%  When describing the pedestrian's behavior from the dashcam images, several essential clues are considered:

% Position Relative to Curb: Observing the pedestrian's position in relation to the curb helps to identify their movement. Initially, they are close to the curb, indicating they have just started crossing.

% Distance Covered: The change in distance between the pedestrian and the curbs on either side of the street across the images indicates the progress of the crossing.

% Body Orientation: The pedestrian's body orientation, particularly the direction they are facing or looking, can suggest awareness of the vehicle. In this case, the pedestrian appears to glance towards the vehicle, indicating awareness of its presence.

% Speed of Movement: Though not directly measurable from still images, the pedestrian's speed can be inferred by how much distance they cover between each frame. A consistent distance covered suggests a steady pace.

% Road Markings: Any visible road markings can be useful to determine if the pedestrian is crossing at a crosswalk or jaywalking. In this series, there doesn't appear to be a crosswalk, which suggests the pedestrian may be crossing at an unmarked location.

% Vehicle's Proximity: The proximity and relative size of the pedestrian in each frame in relation to the vehicle provide context for the pedestrian's behavior in response to oncoming traffic.

% Other Traffic: The presence of other vehicles and their position can affect the pedestrian's behavior. In these images, there doesn’t seem to be immediate traffic that the pedestrian has to navigate around, which may contribute to the seemingly relaxed pace of crossing.

% These clues combined allow for a detailed description of the pedestrian's behavior throughout the sequence of images.
% \end{leftbubbles}
% \begin{rightbubbles}
%     How do you infer the pedestrian's speed between each frame?
% \end{rightbubbles}
% \begin{leftbubbles}
% The inference of a pedestrian's speed between frames in a series of images can be estimated by considering the following factors:
% \begin{itemize}
%     \item Change in Position: By comparing the pedestrian's position across the frames, we can see how much ground they have covered. If the distance covered between frames is consistent, we can infer a steady walking speed.
%     \item Time Interval: If we know the time interval between each frame, we can more accurately estimate the speed. Without this information, we must assume the frames are evenly spaced over time.
%     \item Scale and Reference Points: Using static objects in the images, like the width of the road, lane markings, or parked cars, as reference points can provide a scale to estimate the distance traveled by the pedestrian.
%     \item Pedestrian's Posture and Gait: Observing the posture and stride of the pedestrian can give clues about their speed. For instance, if the pedestrian's legs are captured in a stride, we can infer forward motion.
%     \item Blurring of Image: If there is any motion blur around the pedestrian, it might indicate a quicker pace, but this is not present in clear images.
%     \item Sequence Context: The context of the sequence can offer hints. If a pedestrian is crossing a busy road, they might move faster than if they were crossing a quiet street. However, the presence of a vehicle (in this case, the one with the dashcam) should prompt a quicker crossing, yet the pedestrian appears to be moving at a constant, unhurried pace.
% \end{itemize}
% In the absence of explicit timing information or motion indicators, the estimation of speed from still images remains approximate. The inference is generally based on the change in the pedestrian's position relative to the static environment around them.
% \end{leftbubbles}
% \begin{rightbubbles}
%     if the vehicle is also moving, will the change of pedestrian's position identified between each image be misleading?
% \end{rightbubbles}
% \begin{leftbubbles}
%     Yes, if the vehicle from which the images are being taken is also moving, the apparent movement of the pedestrian in the images could be misleading. This is due to the relative motion between the camera and the pedestrian. The change in the pedestrian's position in the pixel space of the images will be a combination of their own movement and the movement of the vehicle. Here's why:
% \begin{itemize}
%     \item Relative Motion: If the vehicle with the camera is moving, the pedestrian's position will change in the images due to this motion as well as their own.
%     \item Parallax Effect: Objects closer to the camera will appear to move faster across the field of view than objects that are farther away.
%     \item Speed of the Vehicle: The faster the vehicle is moving, the more pronounced the relative motion effect will be.
%     \item Angle of View: If the vehicle is not moving directly towards or away from the pedestrian, the angle of movement also complicates the interpretation of the pedestrian's speed.
%     \item Perspective Changes: As the vehicle moves, the perspective from which the pedestrian is viewed changes, which can affect the apparent speed.
% \end{itemize}
% To accurately determine the pedestrian's speed in such a situation, you would need to account for the speed and direction of the vehicle. Advanced methods such as motion tracking and image stabilization algorithms can help isolate the pedestrian's movement from that of the vehicle. These methods can be complex and require more data than just the images themselves, such as the exact speed of the vehicle, the frame rate of the camera, and the dimensions of the scene.
% \end{leftbubbles}
\end{chatbox}
Another evaluation was done on the WiDEViEW dataset. OpenAI API was used for this evaluation and the language prompt was same as that used for the Quantitative evaluation. A total of 10 frames were input with 10 skipped frames in between. In this image sequence, the pedestrian with red bounding box was on the sidewalk during first 4 frames and started crossing only in the second half of the sequence. The model fails to summarise or detect the change in pedestrian behavior (from sidewalk to crosswalk) suggesting that when the pedestrian is farther away, significant change in action (like moving from sidewalk to crosswalk) is not captured by the model.

\begin{chatbox}[label=chat:bbox_size_wideview,title= Effect of pedestrian size on WiDEVIEW images]
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/seq6_sidewalk.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
    "summary": "In the current 10 frames, \textcolor{red}{the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path.} The pedestrian is walking and not looking towards the ego-vehicle."
     
    "current": 
    "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. 
    "future": 
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
\end{leftbubbles}
\end{chatbox}





==> chats/crossing.tex <==
\subsubsection{Definition of Crossing Road} In this experiment, we presented ChatGPT-4V with an image captured by the front camera of a self-driving vehicle, focusing on a pedestrian's actions. Initially, when asked if the pedestrian was crossing the road, GPT-4V responded negatively. To understand its reasoning, we inquired about its definition of 'road crossing'. The response highlighted that GPT-4V's assessment relies on factors like crosswalks and intersections. However, when we directed its attention to a faded crosswalk where the pedestrian was located, GPT-4V maintained its original stance, albeit with diminished confidence in its last answer. This suggests that GPT-4V's decision-making process might weigh certain visual cues, like the clarity of road markings, more heavily in its analysis.
\\
\begin{chatbox}{}
%\rule{\linewidth}{1pt}
%\begin{figure}[!h]
%\begin{flushright}
 % \includegraphics[width=0.5\textwidth]%{chats/images/crosssing.jpg}
%\end{flushright}
%\end{figure}
\begin{flushright}
\begin{minipage}[t]{0.5\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{chats/images/crosssing.jpg}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
Can you describe this image for me?
\end{rightbubbles}

\begin{leftbubbles}
The image appears to be taken from the perspective of a car's dashboard camera. It shows a street view with a mix of bare trees and a cloudy sky, suggesting it might be late autumn or winter. On the left side, there's a pedestrian sidewalk with a person walking, highlighted by a red outline. In the background, there's a park area with benches and a small structure, possibly a bus stop. The center of the image shows a road with cars parked on the side and one moving in the opposite direction. On the right, there's a distinct building with a red facade and some architectural details, which seems to be a point of interest. A few people are visible near the entrance of this building. There are various road signs indicating traffic directions and restrictions.    
\end{leftbubbles}
\begin{rightbubbles}
Do you think the pedestrian in the red box is trying to cross the road that the ego-vehicle is on?    
\end{rightbubbles}
\begin{leftbubbles}
Based on the image, the pedestrian within the red box appears to be walking parallel to the road that the vehicle (from which the picture is taken) is on, rather than attempting to cross it. The pedestrian's body language and orientation suggest that \textcolor{red}{they are moving along the sidewalk, and there is no clear indication, like a pedestrian crossing, that they are preparing to cross the road at that exact moment.} However, without additional context or a sequence of images showing movement, it's not possible to definitively determine the pedestrian's intentions.    
\end{leftbubbles}
\begin{rightbubbles}
Can you tell me what's the difference between crossing  and walking parallel to the road?    
\end{rightbubbles}
\begin{leftbubbles}
Crossing the road refers to a pedestrian moving from one side of the road to the other, which generally involves traversing the path of vehicular traffic. This action can occur at crosswalks, intersections, or potentially any point along the road, though for safety and legal reasons, crossing is usually done at designated areas.

Walking parallel to the road means the pedestrian is moving in a direction that follows the course of the road, without crossing it. Typically, this is done on a sidewalk or footpath that runs alongside the road. The pedestrian's path of movement does not intersect with the vehicular traffic lanes.

In the image, the pedestrian appears to be walking parallel to the road because their path is along the sidewalk, a space designated for such movement, and there is no indication of them moving towards the traffic lanes that would suggest an attempt to cross.    
\end{leftbubbles}
\begin{rightbubbles}
Is the pedestrian on a crosswalk?    
\end{rightbubbles}
\begin{leftbubbles}
In the provided image, the pedestrian within the red box does not appear to be on a crosswalk. They seem to be walking along the sidewalk, and there are no visible markings on the road that would indicate the presence of a crosswalk at their location. \textcolor{red}{Crosswalks are typically marked by distinct parallel lines, zebra patterns, or other road surface markings}, none of which are evident near the pedestrian in the image.    
\end{leftbubbles}
\begin{rightbubbles}
If you check the left of the pedestrian, there are some zebra patterns. It seems that the zebra patterns are worn down. 
\end{rightbubbles}
\begin{leftbubbles}
Upon closer examination, if there are faded zebra patterns to the left of the pedestrian, then it's possible that this is indeed a worn-down crosswalk. The presence of such patterns, even if they are not clearly visible due to wear or low image quality, would indicate that the pedestrian is at or near a designated crossing area. \textcolor{red}{However, the pedestrian in the image is not directly on the patterns themselves but adjacent to them, which suggests they may be walking parallel to the road rather than actively crossing it at this moment.} Without clearer markings or additional context, it is difficult to conclusively determine the status of the crosswalk and the pedestrian's intentions.    
\end{leftbubbles}
\end{chatbox}

==> chats/cyclist.tex <==
\subsubsection{\textbf{WiDEViEW Dataset}}
For Qualitative evaluation on the WiDEViEW, we focused on three interesting types of scenarios. 

\textbf{Pedestrian}: First type of scenarios consists of pedestrian movements to compare how GPT-4V performs on our dataset in comparison to JAAD and PIE. The language prompt used was same as the one mentioned in the method section and consisted of system, question and format prompt. 

\textbf{Cyclist}: Second type of scenarios consisted of evaluating a cyclist behaviour. Minor changes were made to the prompt replacing "pedestrian" with "cyclist" and replacing the action "walking" with "moving". In terms of movement, cyclist scenario differed from typical pedestrian scenarios as it consisted of movements like walking on the side of the vehicle and overtaking it to eventually cross etc. which offers a different interaction with a vehicle compared to a pedestrian crossing behaviour on a crosswalk.

\textbf{Group}: Third type of scenario involved a more hybrid behaviour consisting of a group of pedestrians, cyclists or both interacting with the vehicle on crosswalks and intersections. Since we did not have the ground truth annotations of groups of pedestrians and cyclists, through this scenario evaluation we tested the GPT-4V capabilities to describe the crosswalk scenario including group identification, group description and group behaviour.


\paragraph{\textbf{Qualitative analysis: WiDEViEW}}
Figure \ref{fig:seq6_uwb} shows the input sequence of 10 frames for one of the pedestrian scenarios considered for evaluation. GPT-4V was tasked to predict pedestrian behavior for the next 5 frames. There was a gap of 10 frames between each of the 10 input frames. 
\begin{figure*}[!h]
    \centering
    \includegraphics[scale=0.35]{images/UWB_data/seq6_v1.png}
    \caption{Pedestrian Scenario from the WiDeView Dataset}
    \label{fig:seq6_uwb}
    \end{figure*}


The response for this scenario is shown in Listing \ref{Resp:seq6}. The response is correct and as expected and matches with the pedestrian behavior. In this case, the first input of the frame (Frame 0) was such that the pedestrian had already stepped down on the crosswalk and started to cross. Listing \ref{Resp:seq6_incorrect} shows the response for a different set of input frames from the same scenario. To avoid redundancy and highlight the differences only the summary, reasoning and future reasoning part of the responses are shown. In this case, the first 4 frames were when pedestrian was still on the sidewalk and stepped on the crosswalk only in the 5th frame. As can be seen from the response, the model fails to summarise or detect the change in pedestrian behavior (from sidewalk to crosswalk). A potential reason for the same can be that in this case vehicle was further away from the pedestrian compared to the previous case and thus the bounding box size was smaller to detect the sidewalk to crosswalk movement in the last 5 frames.

\begin{figure*}[!h]
%\centering
\includegraphics[scale=0.1]{images/UWB_data/cyclist.png} \hspace{-0.98cm}
\includegraphics[scale=0.1]{images/UWB_data/cyclist_cross.png} 
\includegraphics[scale=0.1]{images/UWB_data/cyclist_walk.png} 
\includegraphics[scale=0.1]{images/UWB_data/single_group_2.png}
    \caption{Example frames from various scenarios of the WiDEViEW Dataset. The top 2 figures show 2 frames from the same scenario of an input sequence, where on the left cyclist is ahead of the vehicle and a couple of frames later (on the right) crosses in front of the vehicle. The bottom left frame shows an example input frame from another scenario with a pedestrian walking with a bicycle. The bottom right shows two pedestrians walking on the crosswalk.}
    \label{fig:scenarios_uwb}
\end{figure*}

\begin{listing}
\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{     
   "summary": "In the current 10 frames, the pedestrian within the red box is crossing the road, 
   moving from the right side to the left side of the ego-vehicle's path.
   
   The pedestrian's path intersects with that of the ego-vehicle, and they appear to be walking and looking towards the direction of the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian within the red box is observed to be in different positions on the road across the frames, indicating movement. The direction of the pedestrian's movement is from the right to the left side of the road, and they are facing towards the ego-vehicle, suggesting awareness of the vehicle's presence.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
    "looking": ["looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking"]
  },
  "future": {
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue to cross the road in the next few frames. The pedestrian is expected to keep walking and may or may not look towards the ego-vehicle as they finish crossing.",
    "drive": ["no", "no", "no", "yes", "yes"],
    "crossing": ["crossing", "crossing", "crossing-irrelevant", "crossing-irrelevant", "not-crossing"],
    "action": ["walking", "walking", "walking", "walking", "standing"],
    "looking": ["looking", "not-looking", "not-looking", "not-looking", "not-looking"]
}
\end{minted}
\caption{Response for Pedestrian Scenario from the WiDEViEW Dataset. The response is for the sequence of 10 input frames where the pedestrian starts crossing the road from the first input frame itself.} 
\label{Resp:seq6}
\end{listing}

\begin{listing}
\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path. The pedestrian is walking and not looking towards the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. The pedestrian's body language suggests they are walking and their orientation indicates they are not looking at the ego-vehicle."
  },
  "future": {
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
   ]
  }
}
\end{minted}
\caption{Response for Scenario type 1 from the WiDEViEW Dataset. The response is for the sequence of 10 input frames where for the first half of the sequence, the pedestrian is still on the sidewalk and comes to the crosswalk only in the second half of the sequence} 
\label{Resp:seq6_incorrect}
\end{listing}



Fig. \ref{fig:scenarios_uwb} shows 3 different scenarios from the WiDEViEW dataset that were considered for evaluation. First scenario (top row in Fig. \ref{fig:scenarios_uwb} involves a cyclist which comes in the frame on the left of the ego-vehicle and eventually overtakes the vehicle and crosses in front of it. Another scenario (Bottom left in Fig. \ref{fig:scenarios_uwb}) shows a pedestrian walking with a bicycle. A similar language prompt (shown in green bubble) as the pedestrians was used for both cyclist scenarios with the only change of pedestrian replaced by cyclist and the action of walking was changed to moving. Responses for the two scenarios are shown in Listing \ref{Resp:seq_cyc_} and \ref{Resp:seq_cyc_walking} respectively. 
\begin{listing}[!t]
\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the cyclist within the red box is moving across the crosswalk in a direction that intersects with the ego-vehicle's path. The cyclist is moving and looking in the direction of travel, not towards the ego-vehicle.",
  "current": {
    "reasoning": "The cyclist is observed to be in motion across the frames, moving from the right side of the road towards the left, crossing the path of the ego-vehicle. The cyclist's head orientation suggests they are looking ahead and not towards the ego-vehicle.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving"],
    "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
  },
  "future": {
    "reasoning": "Based on the current trajectory and speed of the cyclist, it is likely that they will continue to cross the road in front of the ego-vehicle. The cyclist is expected to keep moving and may or may not look towards the ego-vehicle as they continue to cross.",
    "drive": ["no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["moving", "moving", "moving", "moving", "moving"],
    "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
  }
}
\end{minted}
\caption{Response for second scenario in Type 2 Scenario, where the cyclist starts on the left side of the vehicle and eventually overtakes to cross in front of the vehicle.} 
\label{Resp:seq_cyc_}
\end{listing}


\begin{listing}

\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the pedestrian within the red box is walking with a bicycle and crossing the road. The pedestrian's path intersects with that of the ego-vehicle, and they are looking towards the direction of the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian is observed to be walking with a bicycle across the crosswalk, which intersects with the ego-vehicle's path. The pedestrian's head orientation and body position suggest they are aware of the ego-vehicle's presence.",
  },
  "future": {
    "reasoning": "Based on the current trajectory and speed of the pedestrian, it is likely that they will continue to cross the road in the next 5 frames. The ego-vehicle should not drive forward very fast to avoid a collision."
   }
\end{minted}
\caption{Response for second scenario in Type 2 Scenario, where a pedestrian walking with a bicycle crosses in front of the vehicle. This shows model's ability to differentiate between cyclist vs pedestrian walking with a bicycle even though the prompt provided was exactly same as the cyclist overtaking scenario.} 
\label{Resp:seq_cyc_walking}
\end{listing}

% \begin{listing}

% \begin{minted}[frame=single,
%                framesep=1mm,
%                linenos=false,
%                xleftmargin=2pt,
%                tabsize=2,
%                fontsize=\footnotesize,
%                breaklines]{js}
% {
% These are {num_frames} ego-vehicle front-camera view images that you can see behind the wheel. \
% More than one pedestrians in close proximity to each other can be termed as a group of pedestrians
% Here are the definitions of the pedestrian group descriptions we are interested in: \
% * Cross: Not-crossing: The group of pedestrian is not crossing the road .\
%         Crossing: The group of pedestrians is actively crossing the road and their path intersects with that of the ego-vehicle.\
%         Crossing-irrelevant: The pedestrian is crossing the road, but their path does not intersect with the ego-vehicle's path, hence it is irrelevant to the vehicle's immediate trajectory.\
% * Action: Whether the group of pedestrian is `walking` or `standing` \
% * Look: This term describes the pedestrian's attention in relation to the ego-vehicle, indicating if the group is 'looking' towards or 'not-looking' (not-facing) away from the direction of the ego-vehicle. \
% By answering the following questions, can you describe the current {num_frames} frames and predict the next {prediction_num} frame behavior of the pedestrian groups separately?                
% Questions: \
% * Can you describe the crosswalk scene in detail and how it changes across {num_frames} frames? \
% * Do you see a group or multiple groups of pedestrians on the road? \
% * How many groups are there and can you tell how many pedestrians are there in each group? \
% * Are there any other vehicles in the scene? \
% * Do any of the other vehicle (if present) occlude the crosswalk view of the ego vehicle? \
% * Can you describe the crossing behaviour of each group ? \
% * Can you describe the action of each group? \
% Please give in JSON format, including the following fields; each field is a list of answers for current {num_frames} frames and future {prediction_num} frames: \
% "summary": "your description for the current  {num_frames}  frames", please be as detailed as possible \
% "current" {{ \
% "reasoning": "your reasoning procedure for describing the behavior of the groups identified in the current {num_frames} frames",
% "drive": ["yes/no"], \
% "crossing": ["not-crossing/crossing/crossing-irrelevant"], \
% "action": ["standing/walking"], \
% "looking": ["not-looking/looking"], \
% }}, \
% "future": {{ \
% "reasoning": "your reasoning procedure for predicting the behavior of the groups of pedestrian  in the future {prediction_num} frames", \
% "drive": ["yes/no"], \
% "crossing": ["not-crossing/crossing/crossing-irrelevant"], \
% "action": ["standing/walking"], \
%  "looking": ["not-looking/looking"],
%                 """}
% }}
% \end{minted}
% \caption{Group Prompt}
% \label{prompt:seq_group}
% \end{listing}
% \begin{listing}

% \begin{minted}[frame=single,
%                framesep=1mm,
%                linenos=false,
%                xleftmargin=2pt,
%                tabsize=2,
%                fontsize=\footnotesize,
%                breaklines]{js}
% {
%   "summary": "The crosswalk scene shows a single group of pedestrians, consisting of two individuals, crossing the road. The group's behavior changes across the 10 frames as they move from one side of the crosswalk to the other. There is one vehicle present in the scene, which does not occlude the crosswalk view for the ego-vehicle.",
%   "current": {
%     "reasoning": "Based on the sequence of images, the group of pedestrians is observed to be crossing the road from the ego-vehicle's right to left. They are walking and looking in the direction of the ego-vehicle, indicating awareness of the vehicle's presence.",
%     "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
%     "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
%     "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
%     "looking": ["looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking"]
%   },
%   "future": {
%     "reasoning": "Assuming the pedestrians maintain their current pace and trajectory, they will likely finish crossing the road in the next few frames. The ego-vehicle should remain stationary until the pedestrians have safely crossed.",
%     "drive": ["no", "no", "no", "yes", "yes"],
%     "crossing": ["crossing", "crossing", "not-crossing", "not-crossing", "not-crossing"],
%     "action": ["walking", "walking", "standing", "standing", "standing"],
%     "looking": ["looking", "not-looking", "not-looking", "not-looking", "not-looking"]
%   }
% }
% \end{minted}
% \caption{Group behaviour single group of two. no bounding box provided. changed prompt. \textcolor{red}{TODO. To avoid repeating keep only summary and reasoning for some of the cases.}} 
% \label{Resp:seq_group}
% \end{listing}
An interesting thing to observe here is that the LLM was able to differentiate between a cyclist vs. a pedestrian walking with a bicycle. This is an important distinction for AV applications as the speed of the road user will be significantly different in both cases thus requiring different navigation responses from the autonomous vehicle. However, in the case of the cyclist LLM incorrectly summarised the cyclist movement as crossing throughout the 10 input frames even though the cyclist is on the left side of the vehicle moving parallel ahead and starts crossing and coming in ego vehicle's path only in the last couple of frames.

Modeling the group behavior of road users is an important aspect of studying vehicle-pedestrian interactions. Detecting groups of road users and predicting the behavior/intent of a group can be particularly beneficial in scenarios where some part of multimodal information about individual pedestrians might be sparse. Additionally, modeling and observing the behavior of a group can potentially lead to better and more ahead-of-time predictions as a group can have richer historical observations than individual pedestrians. To this end, we also evaluated LLM's ability to describe group scenarios. Since we don't have the annotated ground truth bounding boxes of groups, raw frames were input without any bounding box. Additionally, the prompt was modified to include definition of a group as well as additional questions to get details of the group as well as details of the traffic scene. The prompt used is shown in Listing \ref{prompt:seq_group}. Response is shown in Listing \ref{Resp:seq_group}. As seen in response LLM is able to successfully detect the group as well as the number of pedestrians in the group. Additionally, for the future predictions it correctly predicts not crossing for the last 3 frames as it correctly predicts that the two pedestrians are about to finish crossing the road in the next couple of frames.

==> chats/exp_design.tex <==
\begin{center}
\begin{figure*}[h]
\setlength{\tabcolsep}{0pt} % Removes spacing between columns
\begin{tabular}{c c c c c} 
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_0.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_1.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_2.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_3.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_4.jpg}\\
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_5.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_6.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_7.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_8.jpg}&
\includegraphics[width=0.2\textwidth]{chats/images/0_227_1720b/0_227_1720b_9.jpg}\\
\end{tabular} 
\caption{Sequence of annotated images from the JAAD dataset, highlighting a single pedestrian with a red bounding box.}
\label{fig:exp_design_example}
\end{figure*}
\end{center}
For quantitative experiments, we utilize the OPENAI Python API to perform a batch evaluation on JAAD datasets. We task the model with inferring information from $n$ past frames and predicting pedestrian intention for $m$ future frames. Key behaviors we focus on, annotated in the JAAD dataset, include Crossing, Action, and Looking. 

Due to the current limitations of the OPENAI API, our experiment design is constrained to a single prompt format. The key parameters we manipulate are \texttt{num\_frames}, \texttt{prediction\_num}, and \texttt{skip\_num}. The JAAD dataset videos are captured at a frequency of 30 FPS. Our preliminary experiments indicate that the model struggles to discern differences between frames that are too closely spaced. While an ideal experiment would vary \texttt{skip\_num}, API constraints limit us to a batch analysis with ten different \texttt{skip\_num}. Consequently, we set \texttt{num\_frames} to 10 and \texttt{prediction\_num} to 5.

Our prompts are constructed based on best practices (see \cite{BestPracticesPrompt}) and iterative trial-and-error. The initial system message is designed to contextualize the AI’s role as an autonomous vehicle equipped to process front-camera images for pedestrian interaction and capable of outputting JSON files. The prompt is as follows:\\
\begin{minted}[frame=single, framesep=1mm, linenos=false, xleftmargin=2pt, tabsize=2, fontsize=\footnotesize, breaklines]{python}
"You are an autonomous vehicle that uses front-camera images to interact with pedestrians and also a helpful assistant designed to output JSON."
\end{minted}

Subsequently, we input image details along with the definitions of the targeted behaviors for analysis. Rather than requesting predictions for every pedestrian in the image, we focused our inquiry on a single pedestrian, distinguished by a red bounding box (see Fig. \ref{fig:exp_design_example}). This approach, primarily adopted for evaluation purposes, also aligns with standard practices in pedestrian intent prediction research \cite{huangLearningPedestrianActions2023}. Concentrating on one pedestrian at a time helped alleviate difficulties in accurately associating the model's responses with specific individuals in the scene.

The images were entered sequentially and initially we used the definitions provided in the JAAD dataset. However, we soon realized that these definitions were not ideal for the model's understanding and task performance. Consequently, we turned to ChatGPT for help in refining these definitions. This modification led to a noticeable improvement in the model's performance, as the revised definitions were more conducive to its comprehension and predictive capabilities compared to the original ones.\\
\begin{minted}[frame=single, framesep=1mm, linenos=false, xleftmargin=2pt, tabsize=2, fontsize=\footnotesize, breaklines]{python}
f"""These are {num_frames} ego-vehicle front-camera view images that you can see behind the wheel.\
Here are the definitions of the pedestrian behaviors we are interested in: \
* Cross: Not-crossing: The pedestrian is not crossing the road .\
Crossing: The pedestrian is actively crossing the road and their path intersects with that of the ego-vehicle.\
Crossing-irrelevant: The pedestrian is crossing the road, but their path does not intersect with the ego-vehicle's path, hence it is irrelevant to the vehicle's immediate trajectory.\
* Action: Whether the pedestrian is `walking` or `standing` \
* Look: This term describes the pedestrian's attention in relation to the ego-vehicle, indicating if the pedestrian is 'looking' towards or 'not-looking' (not-facing) away from the direction of the ego-vehicle. """
\end{minted}
Our approach to inference and prediction involved posing specific questions to the model. Initially, these questions were directly tied to the three key behaviors we were investigating. However, we encountered a challenge: the model struggled to distinguish between 'crossing' and 'walking along a sidewalk'. To mitigate this issue, we introduced an additional question. This adjustment proved to be somewhat effective, enhancing the model's ability to differentiate between these two behaviors.\\

\begin{minted}[frame=single, framesep=1mm, linenos=false, xleftmargin=2pt, tabsize=2, fontsize=\footnotesize, breaklines]{python}
f"""By answering the following questions, can you describe the current {num_frames} frames and predict the next {prediction_num} frame behavior of the pedestrian within the red box separately?                
Questions: \
* Can you drive forward very fast without hitting the pedestrian within the red box ? \
* Is the pedestrian crossing in front of our car? \
* What's the action (standing/walking) of the pedestrian? \
* Is the pedestrian looking towards the direction of the ego-vehicle (not-looking/looking)?` """
\end{minted} 

In the final step of our procedure, we directed the model to present its responses in a predefined JSON format. This structured output was essential for consistent analysis and interpretation of the results.
We consolidated all the prompts into a single text-based input, followed by a series of image prompts. Given that GPT is a generative model, its outputs can vary with each iteration. To enhance determinism in our experiments, we configured internal parameters of the GPT model, setting 'temperature' to 0 and 'seed' to 0. Additionally, to ensure consistency and reliability, we repeated the same prompt sequence five times and analyzed the responses. 


==> chats/wideview.tex <==
\subsubsection{Effect of Input Frames}
In this scenario, we evaluate GPT-4V capability on pedestrian range of motion change in the input frames and how it impacts the predictions and behaviour summarization, especially if the pedestrian is far away from the vehicle. This evaluation was done on the WiDEViEW dataset. OpenAI API was used for this evaluation and the language prompt was same as that used for the Quantitative evaluation. A total of 10 frames were input with 10 skipped frames in between. The input image sequences with pedestrian annotated in the form of a red bounding box and the corresponding responses are given below. Please note that only the summary, reasoning for current frames and reasoning for future frames are shown as a part of the response. 

For the first image sequence, the response is reasonable and as expected and matches with the pedestrian behavior. In this case, the first input of the frame (Frame 0) was such that the pedestrian had already stepped down on the crosswalk and started to cross.
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/seq6_v1.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": "In the current 10 frames, the pedestrian within the red box is crossing the road, moving from the right side to the left side of the ego-vehicle's path.
   The pedestrian's path intersects with that of the ego-vehicle, and they appear to be walking and looking towards the direction of the ego-vehicle."
"current": 
    "reasoning": "The pedestrian within the red box is observed to be in different positions on the road across the frames, indicating movement. The direction of the pedestrian's movement is from the right to the left side of the road, and they are facing towards the ego-vehicle, suggesting awareness of the vehicle's presence.",
"future": 
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue to cross the road in the next few frames. The pedestrian is expected to keep walking and may or may not look towards the ego-vehicle as they finish crossing.",
\end{leftbubbles}
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/seq6_sidewalk.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
     "summary": "In the current 10 frames, \textcolor{red}{the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path.} The pedestrian is walking and not looking towards the ego-vehicle."
     
  "current": 
    "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. 
  "future": 
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
\end{leftbubbles}
\end{chatbox}
In the second image sequence given above, the pedestrian was on the sidewalk during  first 4 frames and started crossing only in the second half of the sequence. The model fails to summarise or detect the change in pedestrian behavior (from sidewalk to crosswalk) suggesting that when the pedestrian is farther away, significant change in action (like moving from sidewalk to crosswalk) is not captured by the model. \\


\subsubsection{Behaviour analysis comparison with other road users}
We also evaluated the behaviour analysis of GPT-4V for other road users such as cyclists from the image sequences of the WiDEViEW dataset. Minor changes were made to the prompt replacing "pedestrian" with "cyclist" and replacing the action "walking" with "moving". All other API and inpur parameters were same as in the previous case. First image shows two frames from the sequence of 10 images provided to the API where a cyclist starts from left of the vehicle and eventually overtakes it to cross it. The second image row shows a single frame from another sequence where a pedestrian walking with a bicycle is crossing in front of the vehicle. 
An interesting thing to observe here is that the model was able to differentiate between a cyclist vs. a pedestrian walking with a bicycle even though the prompt provided mentioned cyclist only.  However, the model incorrectly summarised the cyclist movement as crossing even though the cyclist is on the left of the vehicle moving parallel ahead and starts crossing in ego vehicle's path only in the last couple of frames. This can be potentially due to distance of the cyclist as well as higher speed compared to pedestrians which led the model to fail
% in discerning the cyclist motion relative to the vehicle.
\begin{chatbox}{}
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[scale=0.07]{images/UWB_data/cyclist.png}
\includegraphics[scale=0.07]{images/UWB_data/cyclist_cross.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": "The cyclist within the red box is moving across the crosswalk in a direction that intersects with the ego-vehicle's path. 
% The cyclist is moving and looking in the direction of travel, not towards the ego-vehicle.",   
"reasoning": "The cyclist is observed to be in motion across the frames, \textcolor{red}{moving from the right side of the road towards the left, crossing the path of the ego-vehicle.} The cyclist's head orientation suggests they are looking ahead and not towards the ego-vehicle."
\end{leftbubbles}
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[scale=0.1]{images/UWB_data/cyclist_walk.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": \textcolor{blue}{The pedestrian within the red box is walking with a bicycle and crossing the road.} The pedestrian's path intersects with that of the ego-vehicle, and they are looking towards the direction of the ego-vehicle."
\end{leftbubbles}
\end{chatbox}

\subsubsection{Multiple bounding boxes}
The next set of evaluations were done interactively through the chatGPT-4. Manually annotated images with multiple bounding boxes of the pedestrians were provided as the input. However no information about the bounding box was given as a part of the chat prompt. The model was able to distinguish between two bounding boxes of different colors as well as correctly detect the number of pedestrians in each box. This chat excerpt also gave us an insight into "urban scene understanding" capability of the model which is discussed in the next subsection. 

\subsubsection{Scene Understanding of Urban environments}
Looking at the chat excerpt further, although the model correctly detected the number of pedestrians in respective bounding boxes, it failed in describing the crossing behaviour of the pedestrians correctly. This was due to the understanding of the sidewalk definition, where the model assumed that a raised concrete with yellow line is a sidewalk rather than a part of the road (in the middle). Even though the initial prompt provided information about the vehicle being on the road, the model failed to summarise the pedestrians as crossing. Additionally since this was a single image input (without any movement information present), the model relied solely on its understanding of the scene to summarise the crossing behaviour and the sunny lighting conditions made its task more difficult.

\begin{chatbox}{}
\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/single_image_multi_ped_annotated.png}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    This is an image taken from front camera of a vehicle moving forward on the road. Can you describe this image?
\end{rightbubbles}
\begin{leftbubbles}
The image appears to be from a vehicle's front camera, capturing a street scene during the daytime. The road is divided by a yellow line, leading to a crosswalk straight ahead. There are trees lining the sidewalk on both sides of the street, providing a sense of an urban or suburban environment. Notably, \textcolor{blue}{there are three sets of pedestrians, each highlighted with a colored rectangular box. Two are marked with a red box, and one with a green box.} \textcolor{red}{The pedestrians are walking on the sidewalk}, indicating a normal, active setting. 
\end{leftbubbles}
% \begin{rightbubbles}
%     Are any of the pedestrians in the path of the vehicle?
% \end{rightbubbles}
% \begin{leftbubbles}
%     No, all the pedestrians shown in the image are on the sidewalk and not in the path of the vehicle. They are walking alongside the road, not across it.
% \end{leftbubbles}
\begin{rightbubbles}
Whats your reasoning behind the statement that pedestrians are walking on the sidewalk?
\end{rightbubbles}
\begin{leftbubbles}
My reasoning is based on the visual information in the image:
\begin{itemize}
\item Sidewalk Positioning: The pedestrians are within the boundaries of the sidewalk, which is separated from the road where the vehicle is likely traveling.
\end{itemize}
\end{leftbubbles}
\begin{rightbubbles}
How is the sidewalk separated from the road? %where the vehicle is likely to be traveling on?
\end{rightbubbles}
\begin{leftbubbles}
\textcolor{red}{The sidewalk is separated from the road by a raised concrete curb}. This curb acts as a physical barrier between the pedestrian space and the area designated for vehicles. Additionally, there is a grassy strip between the curb and the sidewalk, providing further separation. 
% This kind of arrangement is typical in many urban settings, where curbs are used to delineate the boundary between the roadway and the pedestrian walkway for safety and organization. The curb and grassy strip can also be seen as safety features, ensuring that pedestrians have a buffer zone away from the moving traffic.
\end{leftbubbles}
\end{chatbox}

\subsubsection{Group Detection}
This scenario evaluated if the model has the capability to detect groups and categorize individuals and difference of model's explanation compared to more spread out individual pedestrians. This is an interesting scenario because:
\begin{itemize}
    \item Detecting and predicting the behavior or intent of a group of road users can be highly advantageous in situations where there is limited multimodal information available for individual pedestrians.
    \item Modeling the behavior of a group can potentially lead to better and ahead-of-time predictions as a group can have richer historical observations than individual pedestrians.
\end{itemize}
 No pedestrian annotations were provided for this case. GPT-4V initially detected three groups, but later corrected its response to two groups (a pair and a trio). However, model failed to describe the crossing direction of the two groups.
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/group_seq14_no_annotated.jpg}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    Can you describe the behaviours of pedestrians in this image sequence?
\end{rightbubbles}
\begin{leftbubbles}
The image sequence appears to \textcolor{blue}{show a group of pedestrians crossing a street at a crosswalk}. The pedestrians' behavior seems orderly and cautious as they navigate the crosswalk.
\end{leftbubbles}
\begin{rightbubbles}
    Whats your reasoning behind calling the individuals a group?
\end{rightbubbles}
\begin{leftbubbles}
    The term "group" was used to refer to the collection of individuals crossing the street together. These individuals move as a loose collective, each maintaining their own pace yet moving together in the same direction across the crosswalk.
\end{leftbubbles}
\begin{rightbubbles}
    how many distinct groups of individuals do you see in the image sequence?
\end{rightbubbles}
\begin{leftbubbles}
There are three distinct groups of individuals crossing the street:
A pair in dark clothing
A trio composed of two individuals in light tops and one in a dark top, who are also moving together across the crosswalk.
A single individual in a yellow top, separate from the other two groups, crossing at a different pace.
\end{leftbubbles}
\begin{rightbubbles}
    how many individuals do you see walking across the street 
\end{rightbubbles}
\begin{leftbubbles}
In the image sequence, there are five individuals walking across the street:
There is a pair (two individuals) who are walking closely together throughout.
There is another group of three individuals slightly ahead of the pair, one wearing a yellow cap, one in a light-colored top, and one in a darker top.
These five individuals are seen in various stages of crossing the street in the sequence of images
\end{leftbubbles}
\begin{rightbubbles}
    what about the single individual in a yellow top that you mentioned earlier?
\end{rightbubbles}
\begin{leftbubbles}
    I must correct my earlier statement. There is indeed a single individual wearing a yellow top who is part of the group of three initially mentioned. Therefore, there are not two separate groups, but a single group of three individuals that includes the person wearing the yellow top.
Across all images, we see a total of five individuals:
A pair dressed in darker clothing.
A group of three, which includes the individual in the yellow top.
\end{leftbubbles}
\begin{rightbubbles}
    What is the direction of crossing of the pair and the trio?
\end{rightbubbles}
\begin{leftbubbles}
    \textcolor{red}{Both the pair and the trio are crossing from the right to the left relative to the camera's perspective.} As the sequence progresses, they move from the curb on the right side of the frame towards the curb on the left side. 
    % Their shadows fall towards the camera, indicating that the source of light (probably the sun) is behind them, which also supports the direction of movement from right to left as observed from the camera's point of view.
\end{leftbubbles}

\end{chatbox}
\subsubsection{Group behavior analysis}
In this evaluation, we attempted to investigate the following:
\begin{itemize}
    \item Can the model provide any information about group characteristics, \textit{If} it is provided with bounding box annotations and initial information in the prompt about bounding boxes
\end{itemize}
The model incorrectly detected 2 pedestrians instead of 3 in the green bounding box. This was somewhat understandable as one of individuals is occluded in the green box through most of the frames. However with bounding box and prompt information, GPT-4V summarised the direction of crossing of the two groups correctly unlike the previous case. It was also able to provide insights into characteristics like group formation and individual actions of the pedestrians within each group (Example: action of raised arm as a signal of intent to cross). 
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/group_seq14_annotated.jpg}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    This is a time series of six pictures taken from a driving recorder. The chronological order is marked on the corresponding subfigure. As the driver of the car, please describe in detail the behavior of the pedestrians within the red box on the right side of the image and the green box on the left side of the image.
\end{rightbubbles}
\begin{leftbubbles}
The group within the red box on the right side of the image appears to consist of three pedestrians throughout the sequence. The group within the green box on the left side of the image appears to consist of two pedestrians throughout the sequence.
% Both groups of pedestrians obey traffic signals and crosswalk signs, waiting their turn to cross and using the crosswalk as they do.
\end{leftbubbles}
\begin{rightbubbles}
    Are both groups crossing on the crosswalk in front of the vehicle?
\end{rightbubbles}
\begin{leftbubbles}
    Yes, in the sequence of images provided, both groups of pedestrians are crossing the street on the crosswalk in front of the vehicle. \textcolor{blue}{The group in the red box is crossing from the right side to the left side of the vehicle's field of view, while the group in the green box is crossing from the left side to the right side.}
\end{leftbubbles}
\begin{rightbubbles}
    Can you describe the behaviour of each pedestrian in the green box?
\end{rightbubbles}
\begin{leftbubbles}
Pedestrian 1 in the Green Box is  Closer to the driving vehicle and Pedestrian 2 in the Green Box is further from the driving vehicle.
Both pedestrians in the green box are crossing the street together, with the first pedestrian leading the way, and the second pedestrian following closely behind.
\end{leftbubbles}
\begin{rightbubbles}
    Can you describe the behaviour of each pedestrian in the red box?
\end{rightbubbles}
\begin{leftbubbles}
Pedestrian 1 in the Red Box is the Leading pedestrian closest to the camera, Pedestrian 2 in the Red Box is the middle pedestrian. Pedestrian 3 is the trailing pedestrian furthest from the camera. 
Each pedestrian in the red box seems to maintain their relative position within the group as they cross the street
% the leader at the front, the middle pedestrian following, and the trailing pedestrian slightly behind. 
\end{leftbubbles}
\begin{rightbubbles}
    Can you highlight the main differences in group characteristics and the crossing behaviour of each group?
\end{rightbubbles}
\begin{leftbubbles}
Group in Red Box: This group consists of three individuals who are walking in a line, and maintain consistent spacing. Their body language is more aligned and uniform, \textcolor{blue}{indicating a coordinated group movement.}
% with a clear leader setting the pace at the front. 
% They maintain consistent spacing between each other as they cross. 

Group in Green Box:
Comprised of two individuals, they do not exhibit a single-file line as clearly as the group in the red box. \textcolor{blue}{One pedestrian in the green box is notably raising his arm at one point (possibly signaling his intent to the driver to cross), a distinct action not observed in the red box group. Their formation is less structured}, with the second individual walking slightly behind to the side of the first, rather than directly behind.
In summary, the group in the red box seems to have a more linear progression, while the group in the green box displays a looser formation with some individual actions (like the raised arm) that stand out.
\end{leftbubbles}
\end{chatbox}










==> chats/wideview_backup.tex <==
\subsubsection{\textbf{WiDEViEW Dataset}}
For Qualitative evaluation on the WiDEViEW, we focused on three interesting types of scenarios. First type of scenarios consists of pedestrian movements to compare how GPT4V performs on our dataset in comparison to JAAD and PIE. The language prompt used was same as the one mentioned in the method section and consisted of system, question and format prompt. 
Second type of scenarios consisted of evaluating a cyclist behaviour. Minor changes were made to the prompt replacing "pedestrian" with "cyclist" and replacing the action "walking" with "moving". In terms of movement, cyclist scenario differed from typical pedestrian scenarios as it consisted of movements like walking on the side of the vehicle and overtaking it to eventually cross etc. which offers a different interaction with a vehicle compared to a pedestrian crossing behaviour on a crosswalk.
Third type of scenario involved a more hybrid behaviour consisting of a group of pedestrians, cyclists or both interacting with the vehicle on crosswalks and intersections. Since we did not have the ground truth annotations of groups of pedestrians and cyclists, through this scenario evaluation we tested the GPT-4V capabilities to describe the crosswalk scenario including group identification, group description and group behaviour.


\paragraph{Discussion WideView}
Figure \ref{fig:seq6_uwb} shows the input sequence of 10 frames for one of the pedestrian scenarios considered for evaluation. GPT-4V was tasked to predict pedestrian behavior for the next 5 frames. There was a gap of 10 frames between each of the 10 input frames. The response for this scenario is shown in Listing \ref{Resp:seq6}. The response is correct and as expected and matches with the pedestrian behavior. In this case, the first input of the frame (Frame 0) was such that the pedestrian had already stepped down on the crosswalk and started to cross. Listing \ref{Resp:seq6_incorrect} shows the response for a different set of input frames from the same scenario. To avoid redundancy and highlight the differences only the summary, reasoning and future reasoning part of the responses are shown. In this case, the first 4 frames were when pedestrian was still on the sidewalk and stepped on the crosswalk only in the 5th frame. As can be seen from the response, the model fails to summarise or detect the change in pedestrian behavior (from sidewalk to crosswalk). A potential reason for the same can be that in this case vehicle was further away from the pedestrian compared to the previous case and thus the bounding box size was smaller to detect the sidewalk to crosswalk movement in the last 5 frames.

\begin{figure*}[!h]
    \centering
    \includegraphics[scale=0.35]{images/UWB_data/seq6_v1.png}
    \caption{Pedestrian Scenario Type 1 from the WiDeView Dataset}
    \label{fig:seq6_uwb}
    \end{figure*}
\begin{listing}

\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{     
   "summary": "In the current 10 frames, the pedestrian within the red box is crossing the road, 
   moving from the right side to the left side of the ego-vehicle's path.
   
   The pedestrian's path intersects with that of the ego-vehicle, and they appear to be walking and looking towards the direction of the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian within the red box is observed to be in different positions on the road across the frames, indicating movement. The direction of the pedestrian's movement is from the right to the left side of the road, and they are facing towards the ego-vehicle, suggesting awareness of the vehicle's presence.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
    "looking": ["looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking"]
  },
  "future": {
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue to cross the road in the next few frames. The pedestrian is expected to keep walking and may or may not look towards the ego-vehicle as they finish crossing.",
    "drive": ["no", "no", "no", "yes", "yes"],
    "crossing": ["crossing", "crossing", "crossing-irrelevant", "crossing-irrelevant", "not-crossing"],
    "action": ["walking", "walking", "walking", "walking", "standing"],
    "looking": ["looking", "not-looking", "not-looking", "not-looking", "not-looking"]
}
\end{minted}
\caption{Response for Scenario type 1 from the WiDEViEW Dataset. The response is for the sequence of 10 input frames where the pedestrian starts crossing the road from the first input frame itself.} 
\label{Resp:seq6}
\end{listing}

\begin{listing}
\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path. The pedestrian is walking and not looking towards the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. The pedestrian's body language suggests they are walking and their orientation indicates they are not looking at the ego-vehicle."
  },
  "future": {
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
   ]
  }
}
\end{minted}
\caption{Response for Scenario type 1 from the WiDEViEW Dataset. The response is for the sequence of 10 input frames where for the first half of the sequence, the pedestrian is still on the sidewalk and comes to the crosswalk only in the second half of the sequence} 
\label{Resp:seq6_incorrect}
\end{listing}


%\begin{listing}

% \begin{minted}[frame=single,
%                framesep=1mm,
%                linenos=false,
%                xleftmargin=2pt,
%                tabsize=2,
%                fontsize=\footnotesize,
%                breaklines]{js}
% {
%   "summary": "In the current 10 frames, the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path. The pedestrian is walking and not looking towards the ego-vehicle.",
%   "current": {
%     "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. The pedestrian's body language suggests they are walking and their orientation indicates they are not looking at the ego-vehicle.",
%     "drive": ["yes", "yes", "yes", "yes", "yes", "yes", "yes", "yes", "yes", "yes"],
%     "crossing": ["not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing"],
%     "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
%     "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
%   },
%   "future": {
%     "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
%     "drive": ["yes", "yes", "yes", "yes", "yes"],
%     "crossing": ["not-crossing", "not-crossing", "not-crossing", "not-crossing", "not-crossing"],
%     "action": ["walking", "walking", "walking", "walking", "walking"],
%     "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
%   }
% }
% \end{minted}
% \caption{Response for Scenario type 1 from the WiDEViEW Dataset. The response is for the sequence of 10 input frames where for the first half of the sequence, the pedestrian is still on the sidewalk and comes to the crosswalk only in the second half of the sequence} 
% \label{Resp:seq6_incorrect}
% \end{listing}

\begin{figure}
    %\centering
    %\hfill
    \includegraphics[scale=0.2]{images/UWB_data/cyclist.png}
    \includegraphics[scale=0.2]{images/UWB_data/cyclist_cross.png} \\ \\
    \includegraphics[scale=0.2]{images/UWB_data/cyclist_walk.png}
    \includegraphics[scale=0.2]{images/UWB_data/single_group_2.png}
    \caption{Example frames from various scenarios of the WiDEViEW Dataset. The top 2 figures show 2 frames from the same scenario of an input sequence, where on the left cyclist is ahead of the vehicle and a couple of frames later (on the right) crosses in front of the vehicle. The bottom left frame shows an example input frame from another scenario with a pedestrian walking with a bicycle. The bottom right shows two pedestrians walking on the crosswalk.}
    \label{fig:scenarios_uwb}
    \end{figure}

\begin{listing}
Fig. \ref{fig:scenarios_uwb} shows 3 different scenarios from the WiDEViEW dataset that were considered for evaluation. First scenario (top row in Fig. \ref{fig:scenarios_uwb} involves a cyclist which comes in the frame on the left of the ego-vehicle and eventually overtakes the vehicle and crosses in front of it. Another scenario (Bottom left in Fig. \ref{fig:scenarios_uwb}) shows a pedestrian walking with a bicycle. A similar language prompt (shown in green bubble) as the pedestrians was used for both cyclist scenarios with the only change of pedestrian replaced by cyclist and the action of walking was changed to moving. Responses for the two scenarios are shown in Listing \ref{Resp:seq_cyc_} and \ref{Resp:seq_cyc_walking} respectively. An interesting thing to observe here is that the LLM was able to differentiate between a cyclist vs. a pedestrian walking with a bicycle. This is an important distinction for AV applications as the speed of the road user will be significantly different in both cases thus requiring different navigation responses from the autonomous vehicle. However, in the case of the cyclist LLM incorrectly summarised the cyclist movement as crossing throughout the 10 input frames even though the cyclist is on the left side of the vehicle moving parallel ahead and starts crossing and coming in ego vehicle's path only in the last couple of frames.

Modeling the group behavior of road users is an important aspect of studying vehicle-pedestrian interactions. Detecting groups of road users and predicting the behavior/intent of a group can be particularly beneficial in scenarios where some part of multimodal information about individual pedestrians might be sparse. Additionally, modeling and observing the behavior of a group can potentially lead to better and more ahead-of-time predictions as a group can have richer historical observations than individual pedestrians. To this end, we also evaluated LLM's ability to describe group scenarios. Since we don't have the annotated ground truth bounding boxes of groups, raw frames were input without any bounding box. Additionally, the prompt was modified to include definition of a group as well as additional questions to get details of the group as well as details of the traffic scene. The prompt used is shown in Listing \ref{prompt:seq_group}. Response is shown in Listing \ref{Resp:seq_group}. As seen in response LLM is able to successfully detect the group as well as the number of pedestrians in the group. Additionally, for the future predictions it correctly predicts not crossing for the last 3 frames as it correctly predicts that the two pedestrians are about to finish crossing the road in the next couple of frames.
% \textcolor{red}{TODO Alvika: compare prompt responses when you combine pedestrian and cyclist instead of different prompts for both. Check with multiple bounding box colors for multiple pedestrians. Add results when there are multiple groups or bigger groups. Potentially a summary of parameters that were observed to impact this dataset evaluation.}
\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the cyclist within the red box is moving across the crosswalk in a direction that intersects with the ego-vehicle's path. The cyclist is moving and looking in the direction of travel, not towards the ego-vehicle.",
  "current": {
    "reasoning": "The cyclist is observed to be in motion across the frames, moving from the right side of the road towards the left, crossing the path of the ego-vehicle. The cyclist's head orientation suggests they are looking ahead and not towards the ego-vehicle.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving", "moving"],
    "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
  },
  "future": {
    "reasoning": "Based on the current trajectory and speed of the cyclist, it is likely that they will continue to cross the road in front of the ego-vehicle. The cyclist is expected to keep moving and may or may not look towards the ego-vehicle as they continue to cross.",
    "drive": ["no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["moving", "moving", "moving", "moving", "moving"],
    "looking": ["not-looking", "not-looking", "not-looking", "not-looking", "not-looking"]
  }
}
\end{minted}
\caption{Response for second scenario in Type 2 Scenario, where the cyclist starts on the left side of the vehicle and eventually overtakes to cross in front of the vehicle.} 
\label{Resp:seq_cyc_}
\end{listing}

\begin{listing}

\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "In the current 10 frames, the pedestrian within the red box is walking with a bicycle and crossing the road. The pedestrian's path intersects with that of the ego-vehicle, and they are looking towards the direction of the ego-vehicle.",
  "current": {
    "reasoning": "The pedestrian is observed to be walking with a bicycle across the crosswalk, which intersects with the ego-vehicle's path. The pedestrian's head orientation and body position suggest they are aware of the ego-vehicle's presence.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
    "looking": ["looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking"]
  },
  "future": {
    "reasoning": "Based on the current trajectory and speed of the pedestrian, it is likely that they will continue to cross the road in the next 5 frames. The ego-vehicle should not drive forward very fast to avoid a collision.",
    "drive": ["no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["walking", "walking", "walking", "walking", "walking"],
    "looking": ["looking", "looking", "looking", "looking", "looking"]
  }
\end{minted}
\caption{Response for second scenario in Type 2 Scenario, where a pedestrian walking with a bicycle crosses in front of the vehicle. This shows model's ability to differentiate between cyclist vs pedestrian walking with a bicycle even though the prompt provided was exactly same as the cyclist overtaking scenario.} 
\label{Resp:seq_cyc_walking}
\end{listing}

\begin{listing}

\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
These are {num_frames} ego-vehicle front-camera view images that you can see behind the wheel. \
More than one pedestrians in close proximity to each other can be termed as a group of pedestrians
Here are the definitions of the pedestrian group descriptions we are interested in: \
* Cross: Not-crossing: The group of pedestrian is not crossing the road .\
        Crossing: The group of pedestrians is actively crossing the road and their path intersects with that of the ego-vehicle.\
        Crossing-irrelevant: The pedestrian is crossing the road, but their path does not intersect with the ego-vehicle's path, hence it is irrelevant to the vehicle's immediate trajectory.\
* Action: Whether the group of pedestrian is `walking` or `standing` \
* Look: This term describes the pedestrian's attention in relation to the ego-vehicle, indicating if the group is 'looking' towards or 'not-looking' (not-facing) away from the direction of the ego-vehicle. \
By answering the following questions, can you describe the current {num_frames} frames and predict the next {prediction_num} frame behavior of the pedestrian groups separately?                
Questions: \
* Can you describe the crosswalk scene in detail and how it changes across {num_frames} frames? \
* Do you see a group or multiple groups of pedestrians on the road? \
* How many groups are there and can you tell how many pedestrians are there in each group? \
* Are there any other vehicles in the scene? \
* Do any of the other vehicle (if present) occlude the crosswalk view of the ego vehicle? \
* Can you describe the crossing behaviour of each group ? \
* Can you describe the action of each group? \
Please give in JSON format, including the following fields; each field is a list of answers for current {num_frames} frames and future {prediction_num} frames: \
"summary": "your description for the current  {num_frames}  frames", please be as detailed as possible \
"current" {{ \
"reasoning": "your reasoning procedure for describing the behavior of the groups identified in the current {num_frames} frames",
"drive": ["yes/no"], \
"crossing": ["not-crossing/crossing/crossing-irrelevant"], \
"action": ["standing/walking"], \
"looking": ["not-looking/looking"], \
}}, \
"future": {{ \
"reasoning": "your reasoning procedure for predicting the behavior of the groups of pedestrian  in the future {prediction_num} frames", \
"drive": ["yes/no"], \
"crossing": ["not-crossing/crossing/crossing-irrelevant"], \
"action": ["standing/walking"], \
 "looking": ["not-looking/looking"],
                """}
}}
\end{minted}
\caption{Group Prompt}
\label{prompt:seq_group}
\end{listing}




\begin{listing}

\begin{minted}[frame=single,
               framesep=1mm,
               linenos=false,
               xleftmargin=2pt,
               tabsize=2,
               fontsize=\footnotesize,
               breaklines]{js}
{
  "summary": "The crosswalk scene shows a single group of pedestrians, consisting of two individuals, crossing the road. The group's behavior changes across the 10 frames as they move from one side of the crosswalk to the other. There is one vehicle present in the scene, which does not occlude the crosswalk view for the ego-vehicle.",
  "current": {
    "reasoning": "Based on the sequence of images, the group of pedestrians is observed to be crossing the road from the ego-vehicle's right to left. They are walking and looking in the direction of the ego-vehicle, indicating awareness of the vehicle's presence.",
    "drive": ["no", "no", "no", "no", "no", "no", "no", "no", "no", "no"],
    "crossing": ["crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing", "crossing"],
    "action": ["walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking", "walking"],
    "looking": ["looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking", "looking"]
  },
  "future": {
    "reasoning": "Assuming the pedestrians maintain their current pace and trajectory, they will likely finish crossing the road in the next few frames. The ego-vehicle should remain stationary until the pedestrians have safely crossed.",
    "drive": ["no", "no", "no", "yes", "yes"],
    "crossing": ["crossing", "crossing", "not-crossing", "not-crossing", "not-crossing"],
    "action": ["walking", "walking", "standing", "standing", "standing"],
    "looking": ["looking", "not-looking", "not-looking", "not-looking", "not-looking"]
  }
}
\end{minted}
\caption{Group behaviour single group of two. no bounding box provided. changed prompt. \textcolor{red}{TODO. To avoid repeating keep only summary and reasoning for some of the cases.}} 
\label{Resp:seq_group}
\end{listing}

==> chats/wideview_backup_latest.tex <==
\subsubsection{Effect of Input Frames}
In this scenario, we evaluate GPT-4V capability on pedestrian range of motion change in the input frames and how it impacts the predictions and behaviour summarization, especially if the pedestrian is far away from the vehicle. This evaluation was done on the WiDEViEW dataset. OpenAI API was used for this evaluation and the language prompt was same as that used for the Quantitative evaluation. A total of 10 frames were input with 10 skipped frames in between. The input image sequences with pedestrian annotated in the form of a red bounding box and the corresponding responses are given below. Please note that only the summary, reasoning for current frames and reasoning for future frames are shown as a part of the response. 

For the first image sequence, the response is reasonable and as expected and matches with the pedestrian behavior. In this case, the first input of the frame (Frame 0) was such that the pedestrian had already stepped down on the crosswalk and started to cross. . 
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{0.8\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/seq6_v1.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": "In the current 10 frames, the pedestrian within the red box is crossing the road, moving from the right side to the left side of the ego-vehicle's path.
   The pedestrian's path intersects with that of the ego-vehicle, and they appear to be walking and looking towards the direction of the ego-vehicle."
"current": 
    "reasoning": "The pedestrian within the red box is observed to be in different positions on the road across the frames, indicating movement. The direction of the pedestrian's movement is from the right to the left side of the road, and they are facing towards the ego-vehicle, suggesting awareness of the vehicle's presence.",
"future": 
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue to cross the road in the next few frames. The pedestrian is expected to keep walking and may or may not look towards the ego-vehicle as they finish crossing.",
\end{leftbubbles}
\begin{flushright}
\begin{minipage}[t]{0.8\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/seq6_sidewalk.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
     "summary": "In the current 10 frames, \textcolor{red}{the pedestrian within the red box is not crossing the road and does not intersect with the ego-vehicle's path.} The pedestrian is walking and not looking towards the ego-vehicle."
     
  "current": 
    "reasoning": "The pedestrian within the red box is observed to be on the sidewalk, maintaining a consistent path that does not intersect with the vehicle's trajectory. 
  "future": 
    "reasoning": "Based on the current trajectory and behavior of the pedestrian, it is likely that they will continue walking along the sidewalk without crossing the road or looking towards the ego-vehicle."
\end{leftbubbles}
\end{chatbox}
In the second image sequence given above, the pedestrian was on the sidewalk during  first 4 frames and started crossing only in the second half of the sequence. The model fails to summarise or detect the change in pedestrian behavior (from sidewalk to crosswalk) suggesting that when the pedestrian is farther away, significant change in action (like moving from sidewalk to crosswalk) is not captured by the model. \\


\subsubsection{Behaviour analysis comparison with other road users}
We also evaluated the behaviour analysis of GPT-4V for other road users such as cyclists from the image sequences of the WiDEViEW dataset. Minor changes were made to the prompt replacing "pedestrian" with "cyclist" and replacing the action "walking" with "moving". All other API and inpur parameters were same as in the previous case. First image shows two frames from the sequence of 10 images provided to the API where a cyclist starts from left of the vehicle and eventually overtakes it to cross it. The second image row shows a single frame from another sequence where a pedestrian walking with a bicycle is crossing in front of the vehicle. 
An interesting thing to observe here is that the model was able to differentiate between a cyclist vs. a pedestrian walking with a bicycle even though the prompt provided mentioned cyclist only.  However, in the case of the cyclist, the model incorrectly summarised the cyclist movement as crossing throughout the 10 input frames even though the cyclist is on the left side of the vehicle moving parallel ahead and starts crossing and coming in ego vehicle's path only in the last couple of frames. This can be potentially due to distance of the cyclist as well as higher speed compared to pedestrians which led the model to fail in discerning the cyclist motion relative to the vehicle.
\begin{chatbox}{}
\begin{flushright}
\begin{minipage}[t]{0.7\linewidth}
\vspace*{0pt}
\includegraphics[width=0.5\linewidth]{images/UWB_data/cyclist.png}
\includegraphics[width=0.5\linewidth]{images/UWB_data/cyclist_cross.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": "In the current 10 frames, the cyclist within the red box is moving across the crosswalk in a direction that intersects with the ego-vehicle's path. The cyclist is moving and looking in the direction of travel, not towards the ego-vehicle.",   "reasoning": "The cyclist is observed to be in motion across the frames, \textcolor{red}{moving from the right side of the road towards the left, crossing the path of the ego-vehicle.} The cyclist's head orientation suggests they are looking ahead and not towards the ego-vehicle."
\end{leftbubbles}
\begin{flushright}
\begin{minipage}[t]{0.4\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/cyclist_walk.png}
\end{minipage}
\end{flushright}
\begin{leftbubbles}
"summary": In the current 10 frames, \textcolor{blue}{the pedestrian within the red box is walking with a bicycle and crossing the road.} The pedestrian's path intersects with that of the ego-vehicle, and they are looking towards the direction of the ego-vehicle."
\end{leftbubbles}
\end{chatbox}

\subsubsection{Multiple bounding boxes}
The next set of evaluations were done interactively through the chatGPT-4. Manually annotated images with multiple bounding boxes of the pedestrians were provided as the input. However no information about the bounding box was given as a part of the chat prompt as shown below. The model was able to distinguish between two bounding boxes of different colors as well as correctly detect the number of pedestrians in each box. This chat excerpt also gave us an insight into "urban scene understanding" capability of the model which is discussed in the next subsection. 

\subsubsection{Scene Understanding of Urban environments}
As mentioned in the previous subsection, the below chat excerpt also provided an insight into the urban scene understanding of the model. Although the model correctly detected the number of pedestrians in respective bounding boxes, it failed in describing the crossing behaviour of the pedestrians correctly. Upon further investigation in the form of prompts, this was due to the understanding of the sidewalk definition, where the model assumed that a raised concrete with yellow line is a sidewalk rather than a part of the road (in the middle). Even though the initial prompt provided information about the vehicle being on the road, the model failed to summarise the pedestrians as crossing due to incorrect understanding of the scene. Additionally since this was a single image input (without any bounding box movement information present), the model relied solely on its understanding of the scene to summarise the crossing behaviour and the sunny lighting conditions seen in the frame made its task more difficult.

\begin{chatbox}{}
\begin{flushright}
\begin{minipage}[t]{0.5\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/single_image_multi_ped_annotated.png}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    This is an image taken from front camera of a vehicle moving forward on the road. Can you describe this image?
\end{rightbubbles}
\begin{leftbubbles}
The image appears to be a still shot from a vehicle's front camera, capturing a street scene during the daytime. The road is divided by a yellow line, leading to a crosswalk straight ahead. There are trees lining the sidewalk on both sides of the street, providing a sense of an urban or suburban environment. Notably, \textcolor{blue}{there are three sets of pedestrians, each highlighted with a colored rectangular box. Two are marked with a red box, and one with a green box.} \textcolor{red}{The pedestrians are walking on the sidewalk}, indicating a normal, active setting. 
\end{leftbubbles}
% \begin{rightbubbles}
%     Are any of the pedestrians in the path of the vehicle?
% \end{rightbubbles}
% \begin{leftbubbles}
%     No, all the pedestrians shown in the image are on the sidewalk and not in the path of the vehicle. They are walking alongside the road, not across it.
% \end{leftbubbles}
\begin{rightbubbles}
Whats your reasoning behind the statement that pedestrians are walking on the sidewalk?
\end{rightbubbles}
\begin{leftbubbles}
My reasoning is based on the visual information provided in the image:
\begin{itemize}
\item Sidewalk Positioning: The pedestrians are within the boundaries of the sidewalk, which is separated from the road where the vehicle is likely traveling.
\end{itemize}
\end{leftbubbles}
\begin{rightbubbles}
How is the sidewalk separated from the road where the vehicle is likely to be traveling on?
\end{rightbubbles}
\begin{leftbubbles}
In the image, \textcolor{red}{the sidewalk is separated from the road by a raised concrete curb}. This curb acts as a physical barrier between the pedestrian space and the area designated for vehicles. Additionally, there is a grassy strip between the curb and the sidewalk, providing further separation. 
% This kind of arrangement is typical in many urban settings, where curbs are used to delineate the boundary between the roadway and the pedestrian walkway for safety and organization. The curb and grassy strip can also be seen as safety features, ensuring that pedestrians have a buffer zone away from the moving traffic.
\end{leftbubbles}
\end{chatbox}

\subsubsection{Group Detection}
This scenario evaluated if the model has the capability to detect groups and categorize individuals into it and how does model's explanation differ in this case compared to more spread out individual pedestrians. This is an interesting scenario because:
\begin{itemize}
    \item Detecting groups of road users and predicting the behavior/intent of a group can be particularly beneficial in scenarios where some part of multimodal information about individual pedestrians might be sparse.
    \item Additionally, modeling and observing the behavior of a group can potentially lead to better and more ahead-of-time predictions as a group can have richer historical observations than individual pedestrians.
\end{itemize}
 No pedestrian annotations were provided as a part of this sequence. GPT-4V initially detected three groups, but later corrected its response to two groups (a pair and a trio). However, model failed to describe the crossing direction of the two groups correctly.
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{0.5\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/group_seq14_no_annotated.png}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    Can you describe the behaviours of pedestrians in this image sequence?
\end{rightbubbles}
\begin{leftbubbles}
The image sequence appears to \textcolor{blue}{show a group of pedestrians crossing a street at a crosswalk}. Throughout the sequence, the pedestrians' behavior seems orderly and cautious as they navigate the crosswalk.
\end{leftbubbles}
\begin{rightbubbles}
    Whats your reasoning behind calling the individuals a group?
\end{rightbubbles}
\begin{leftbubbles}
    The term "group" was used to refer to the collection of individuals crossing the street together in the image sequence. These individuals move as a loose collective, each maintaining their own pace yet moving together in the same direction across the crosswalk.
\end{leftbubbles}
\begin{rightbubbles}
    how many distinct groups of individuals do you see in the image sequence?
\end{rightbubbles}
\begin{leftbubbles}
    There are three distinct groups of individuals crossing the street, each at different stages of crossing:

A pair in dark clothing, moving together across the crosswalk in each frame.
A trio composed of two individuals in light tops and one in a dark top, who are also moving together across the crosswalk.
A single individual in a yellow top, who is separate from the other two groups and is crossing the street at a different pace.
\end{leftbubbles}
\begin{rightbubbles}
    how many individuals do you see walking across the street 
\end{rightbubbles}
\begin{leftbubbles}
    In the image sequence, there are five individuals walking across the street. Here's the breakdown:

There is a pair (two individuals) dressed in darker clothing who are walking closely together throughout the sequence.
There is another group of three individuals slightly ahead of the pair, one wearing a yellow cap, one in a light-colored top, and one in a darker top.
These five individuals are seen in various stages of crossing the street in the sequence of images
\end{leftbubbles}
\begin{rightbubbles}
    what about the single individual in a yellow top that you mentioned earlier?
\end{rightbubbles}
\begin{leftbubbles}
    Upon reviewing the image sequence again, I must correct my earlier statement. There is indeed a single individual wearing a yellow top who is part of the group of three initially mentioned. Therefore, there are not two separate groups (a trio and a single individual in a yellow top), but rather a single group of three individuals that includes the person wearing the yellow top.

To summarize, across all images, we see a total of five individuals:

A pair dressed in darker clothing.
A group of three, which includes the individual in the yellow top.
\end{leftbubbles}
\begin{rightbubbles}
    What is the direction of crossing of the pair and the trio?
\end{rightbubbles}
\begin{leftbubbles}
    In the image sequence, both the pair and the trio are crossing from the right to the left relative to the camera's perspective. You can tell because as the sequence progresses, they move from the curb on the right side of the frame towards the curb on the left side. Their shadows fall towards the camera, indicating that the source of light (probably the sun) is behind them, which also supports the direction of movement from right to left as observed from the camera's point of view.
\end{leftbubbles}

\end{chatbox}
\subsubsection{Group behavior analysis}
In this evaluation, we attempted to investigate the following:
\begin{itemize}
    \item What additional information can the provide about group characteristics, if it is provided with annotations of the bounding boxes and initial information in the prompt about the bounding boxes.
\end{itemize}
The model incorrectly detected 2 pedestrians instead of 3 in the green bounding box. This was somewhat understandable as the second individual is occluded by the first individual in the green box through most of the frames. However with bounding box and prompt information, GPT-4V summarised the direction of crossing of the two groups correctly unlike the previous case. Surprisingly, it was able to characteristics like group formation and individual actions of the pedestrians within each group (Example: action of raised arm as a signal of intent to cross). 
\begin{chatbox}{}

\begin{flushright}
\begin{minipage}[t]{0.5\linewidth}
\vspace*{0pt}
\includegraphics[width=\linewidth]{images/UWB_data/group_seq14_annotated.png}
\end{minipage}
\end{flushright}
\begin{rightbubbles}
    This is a time series of six pictures taken from a driving recorder. The chronological order is marked on the corresponding subfigure. As the driver of the car, please describe in detail the behavior of the pedestrians within the red box on the right side of the image and the green box on the left side of the image.
\end{rightbubbles}
\begin{leftbubbles}
The group within the red box on the right side of the image appears to consist of three pedestrians throughout the sequence. The group within the green box on the left side of the image appears to consist of two pedestrians throughout the sequence.
Both groups of pedestrians obey traffic signals and crosswalk signs, waiting their turn to cross and using the crosswalk as they do. T
\end{leftbubbles}
\begin{rightbubbles}
    Are both groups crossing on the crosswalk in front of the vehicle?
\end{rightbubbles}
\begin{leftbubbles}
    Yes, in the sequence of images provided, both groups of pedestrians are crossing the street on the crosswalk in front of the vehicle. \textcolor{blue}{The group in the red box is crossing from the right side to the left side of the vehicle's field of view, while the group in the green box is crossing from the left side to the right side.}
\end{leftbubbles}
\begin{rightbubbles}
    Can you describe the behaviour of each pedestrian in the green box?
\end{rightbubbles}
\begin{leftbubbles}
Pedestrian 1 in the Green Box is  Closer to the driving vehicle and Pedestrian 2 in the Green Box is further from the driving vehicle.
Both pedestrians in the green box are crossing the street together, with one slightly ahead of the other. The first pedestrian seems to be leading the way, with the second pedestrian following closely behind.
\end{leftbubbles}
\begin{rightbubbles}
    Can you describe the behaviour of each pedestrian in the red box?
\end{rightbubbles}
\begin{leftbubbles}
Pedestrian 1 in the Red Box is the Leading pedestrian closest to the camera, Pedestrian 2 in the Red Box is the middle pedestrian. Pedestrian 3 is the trailing pedestrian furthest from the camera. 

Each pedestrian in the red box seems to maintain their relative position within the group as they cross the street: the leader at the front, the middle pedestrian following, and the trailing pedestrian slightly behind. 
\end{leftbubbles}
\begin{rightbubbles}
    Can you highlight the main differences in group characteristics and the crossing behaviour of each group?
\end{rightbubbles}
\begin{leftbubbles}
Group in Red Box: This group consists of three individuals who are walking in a line, with a clear leader setting the pace at the front. They maintain consistent spacing between each other as they cross. Their body language is more aligned and uniform, \textcolor{blue}{indicating a coordinated group movement.}

Group in Green Box:
Comprised of two individuals, they do not exhibit a single-file line as clearly as the group in the red box. \textcolor{blue}{One pedestrian in the green box is notably raising his arm at one point (possibly signaling his intent to the driver to cross), a distinct action not observed in the red box group. Their formation is less structured}, with the second individual walking slightly behind to the side of the first, rather than directly behind.
In summary, the group in the red box seems to have a more organized and linear progression across the crosswalk, while the group in the green box displays a looser formation with some individual actions (like the raised arm) that stand out.
\end{leftbubbles}
\end{chatbox}










==> sections/related_work.tex <==
\section{related work}
\subsection{Pedestrian Behavior Prediction Methods}


\subsection{Vision Language Model for Autonomous Driving}




